Barriers to Welfare Maximization with No-Regret Learning

A celebrated result in the interface of online learning and game theory guarantees that the repeated interaction of no-regret players leads to a coarse correlated equilibrium (CCE) -- a natural game-theoretic solution concept. Despite the rich history of this foundational problem and the tremendous interest it has received in recent years, a basic question still remains open: how many iterations are needed for no-regret players to approximate an equilibrium? In this paper, we establish the first computational lower bounds for that problem in two-player (general-sum) games under the constraint that the CCE reached approximates the optimal social welfare (or some other natural objective). From a technical standpoint, our approach revolves around proving lower bounds for computing a near-optimal $T$-sparse CCE -- a mixture of $T$ product distributions, thereby circumscribing the iteration complexity of no-regret learning even in the centralized model of computation. Our proof proceeds by extending a classical reduction of Gilboa and Zemel [1989] for optimal Nash to sparse (approximate) CCE. In particular, we show that the inapproximability of maximum clique precludes attaining any non-trivial sparsity in polynomial time. Moreover, we strengthen our hardness results to apply in the low-precision regime as well via the planted clique conjecture.

==> text/eth.tex <==
\subsection{ETH Hardness}

We will now extend the previous result under the \emph{exponential time hypothesis (ETH)}~\citep{Impagliazzo01:Complexity}, which postulates that any (deterministic) algorithm for solving 3SAT on $n$ variables requires $2^{\Omega(n)}$ time. ETH was used to prove lower bounds for the problem of computing an approximate Nash equilibrium with near-optimal welfare by~\citet{Braverman15:Approximating}. Here, we rely on the subsequent approach of~\citet{Deligkas18:Inapproximability} (to a large extent, we adhere to their notation in our exposition below). 

\paragraph{Two-prover games} We begin by recalling the definition of a \emph{two-prover game}~\citep{Aaronson14:AM}.

\begin{definition}[Two-prover game]
    A \emph{two-prover game} $\cT$ is defined by a tuple $(X, Y, A, B, \cD, V)$, where
    \begin{itemize}
        \item $X$ and $Y$ are finite sets of \emph{questions};
        \item $A$ and $B$ are finite sets of \emph{answers};
        \item $\cD$ is a probability distribution over $X \times Y$; and
        \item $V : X \times Y \times A \times B \to \{0, 1 \}$ is a \emph{verification function}.
    \end{itemize}
\end{definition}

The underlying game is played between two players, say $\merone$ and $\mertwo$, and an arbiter called $\arthur$. The game commences by $\arthur$ drawing a question pair $X \times Y \ni (x, y) \sim \cD$ (according to $\cD$). $\arthur$ then sends $x$ to $\merone$ and $y$ to $\mertwo$---$\merone$ does not know $y$ and $\mertwo$ does not know $x$, whereupon $\merone$ selects an answer $a \in A$ and $\mertwo$ an answer $b \in B$, which are transmitted back to $\arthur$. $\arthur$ then computes the value $u \defeq V(x, y, a, b)$, and each player receives a utility of $u$---that is, $\merone$ and $\mertwo$ share identical interests. The size of the game, denoted by $|\cT|$, is the number of entries needed to represent $V$ in tabular form.

A \emph{strategy} for $\merone$ is a function $S_1 \ni s_1 : X \to A$ mapping questions to answers; similarly, a function for $\mertwo$ is a function $S_2 \ni s_2 : Y \to B$. The (expected) utility of the game under a pair of strategies $(s_1, s_2) \times S_1 \times S_2$ reads
\[
    u(\cT, s_1, s_2) \defeq \E_{ (x, y) \sim \cD} [ V(x, y, s_1(x), s_2(y)].
\]
In particular, the \emph{value} of the game, denoted by $v(\cT)$, is the expected utility obtained under optimal play:
\[
    v(\cT) \defeq \max_{ (\sstar_1, \sstar_2) \in S_1 \times S_2} u(\cT, \sstar_1, \sstar_2).
\]

\paragraph{Free games} A two-prover game is a \emph{free game} if $\cD$ is a \emph{product} distribution over $X \times Y$; that is, there is no correlation between the question sent to $\merone$ and the question sent to $\mertwo$. In this context, the problem $\freegame_\delta$ is defined as follows. We are given as input a parameter $\delta > 0$ and a free two-prover game $\cT$, and the goal is to compute a value $u$ such that $| u - v(\cT) | \leq \delta$.

\paragraph{Hardness of approximating free games} Unlike general two-prover games, free games admit a quasipolynomial-time algorithm~\citep{Aaronson14:AM} (\emph{cf.} \citep{Lipton03:Playing}), but that cannot be significantly improved under ETH. In particular, we will use the following result extracted from~\citep{Babichenko16:Can}, presented in the form below by~\citet{Deligkas18:Inapproximability}.

\begin{theorem}[\citep{Deligkas18:Inapproximability, Babichenko16:Can}]
    \label{theorem:inapprox-free}
    Assuming ETH, there is a sufficiently small constant $\delta$ below which $\freegame_\delta$ cannot be solved faster than $N^{\tilO(\log N)}$, even when the question sets have size $O(\log N)$.
\end{theorem}

Above, we use the notation $\tilO(\log N) = O( \log N / ( \log \log N )^c )$ for some constant $c$.

\paragraph{The reduction} Suppose now that we are given a free game $\cF$ such that each question set has size $O(\log |\cF|)$ (which suffices for the quasipolynomial hardness of \Cref{theorem:inapprox-free}). We will use $\cF$ to construct a two-player game $\cG$ with the following properties.
\begin{itemize}
    \item If $v(\cF) = 1$, then there is a Nash equilibrium in $\cG$ with social welfare $1$.
    \item If $v(\cF) < 1 - \delta$, any $T$-sparse CCE in $\cG$ attains a social welfare of at most $1 - $ \todo{To be filled}.
\end{itemize}

In particular, we define $\cG$ from $\cF$ as follows.

\begin{equation}
    \mat{R} \defeq 
    \frac{1}{2}  
    \begin{pmatrix}
       \mat{A} & - \mat{D}_y \\
        \mat{D}_x & \mat{0}
    \end{pmatrix}
    \text{ and }
    \mat{C} \defeq
    \frac{1}{2} 
    \begin{pmatrix}
       \mat{A} & \mat{D}_y \\
        - \mat{D}_x & \mat{0}
    \end{pmatrix},
\end{equation}
where we have defined the following matrices.
\begin{itemize}
    \item Each row of matrix $\mat{A}$ represents a pair $(x, a) \in X \times A$ and each column a pair $(y, b) \in Y \times B$, so that $\mat{A}_{ (x,a), (y, b)}$ is given by $V(x, y, a, b)$.
    \item $\mat{D}_x$ is defined as follows. Let $\mathcal{H}$ be the set of all functions of the form $f : Y \to \{0, 1\}$ such that $f(y) = 1$ for exactly half of the elements in $Y$ (without any loss, we can assume that $|Y|$ is even). $\mat{D}_x$ then has $|Y \times B|$ columns and $|\mathcal{H}|$ rows, so that for all $f \in \mathcal{H}$ and $(y, b) \in Y \times B$ we have
    \[
        (\mat{D}_x)_{f, (y,b)} = 
        \begin{cases}
        \frac{4k}{1 + 4 g \delta} & \text{if } f(y) = 1,\\
        0 & \text{otherwise}.
        \end{cases}
    \]
    (This is based on an earlier construction due to~\citet{Feder07:Approximating}.)
    \item $\mat{D}_y$ is defined symmetrically with respect to Player $y$.
\end{itemize}

Because $|X|, |Y| \leq O(\log |\cF|)$, the size of $\cG$ is polynomial in $|\cF|$, so the above reduction is polynomial.

\paragraph{Completeness} Let us assume that $v(\cF) = 1$. We need to prove that there is a Nash equilibrium in $\cG = \cG(\cF)$ with social welfare $1$.

\begin{proof}
    Let us consider a pair of optimal strategies $(\sstar_1, \sstar_2) \in S_1 \times S_2$ in $\cF$. We then define
    \[
        \vxstar_{x, a} \defeq 
        \begin{cases}
        \frac{1}{|X|} & \text{if } \sstar_1(x) = a,\\
        0 & \text{otherwise}.
        \end{cases}
    \]
    And
    \[
        \vystar_{y, b} \defeq 
        \begin{cases}
        \frac{1}{|Y|} & \text{if } \sstar_2(y) = b,\\
        0 & \text{otherwise}.
        \end{cases}
    \]
    Given that $\E_{(x, y) \sim \cD} V(x, y, \sstar_1(x), \sstar_2(y)) = 1$, it follows that under $(\vxstar, \vystar)$ each player obtains a utility of $1/2$. Next, we will prove that $(\vxstar, \vystar)$ is a Nash equilibrium of $\cG$. By symmetry, it suffices to consider deviations of Player $y$. In particular, it suffices to bound the deviation benefit from selecting a column from $\mat{D}_y$. \todo{Make sure that there consistency between $k$ and the fraction of elements of $Y$ on which $f$ is activated; the current proof is not consistent.}
\end{proof}

\paragraph{Soundness} Suppose now that $v(\cF) < 1 - \delta$, and consider an approximate $T$-sparse CCE of $\cG$. We will show that it must have social welfare at most $\approx 1 - \delta$.

\begin{lemma}[Informal]
    \label{lemma:onlyA}
    If $\sw(\vmu) \approx 1$, then $\vmu$ must place almost all probability mass on the submatrix corresponding to $\mat{A}$. We can thus transfer all most to that component with a small degradation in the approximation quality.
\end{lemma}

Indeed, the maximum social welfare in $\cG$ is $1$, and every entry outside of the component corresponding to $\mat{A}$ has $0$ welfare, implying the statement above.

We now construct a two-prover game using $(\vx^{(t)}, \vy^{(t)})$, for any $t \in [T]$. First, we define $\vx' \defeq \sum_{a \in A} \vx^{(t)}_{x, a}$ and $\vy' \defeq \sum_{b \in B} \vy^{(t)}_{y, b}$, where we note that $\| \vx' \|_1 = 1$ and $\| \vy' \|_1 = 1$. We now define $\cT \defeq (X, Y, A, B, \cD, V)$, where $\cD$ is the product distribution $\vx' \otimes \vy'$. 

Now, we can use $(\vx^{(t)}, \vy^{(t)})$ to obtain strategies for $\merone$ and $\mertwo$ in $\cT$ as follows. We first note that one can assume that for each question $x \in X$ there is exactly one answer $a \in A$ such that $\vx^{(t)}(x, a) > 0$, for otherwise one can safely shift the probability mass between them. \todo{check this} So, we define the strategy of $\merone$ as follows. For each question $x \in X$, $s_1 = s_1(\vx^{(t)}) $ selects the unique answer $a \in A$ such that $\vx^{(t)}(x, a) > 0$. The strategy for $\mertwo$ is defined symmetrically. We first relate the utility in $\mat{T}$ under $(s_1, s_2)$ with the utility in $\cG$ under $(\vx^{(t)}, \vy^{(t)})$. In particular, because of~\Cref{lemma:onlyA} they are basically equivalent.

Next, we need to show that $\vx'$ and $\vy'$ are close to uniform over the questions. 

==> text/proofs.tex <==
\section{Omitted Proofs}
\label{sec:proofs}

In this section, we provide the proofs omitted from the main body.

\iffalse

\subsection{Proof of Theorem~\ref{theorem:algorithm1}}
\label{appendix:proof1}

We begin with the proof of~\Cref{theorem:algorithm1}. It mostly boils down to~\Cref{lemma:optimalCCE,lemma:bad-mass,lemma:small-prob,lemma:induced-clique}, which are restated and proven below.

\optimalCCE*

\begin{proof}
    Let $K \subseteq V$ denote a clique in $G$ of size $k$, which is assumed to exist. We construct a mixture of product distributions as follows. We partition $K$ into $T$ (disjoint) subsets $K^{(1)}, K^{(2)}, \dots, K^{(T)}$, each of size $k/T$. For each $t \in [T]$, we define $\vx^{(t)} \defeq \vy^{(t)} \defeq \uni(K^{(t)})$, that is, the uniform distribution over $K^{(t)}$. Then, we define $\vmu \defeq \frac{1}{T} \sum_{t=1}^T \vx^{(t)} \otimes \vy^{(t)}$.

    We first claim that $\vmu$ attains a welfare of $1 + \gamma T/k$. Indeed, by the above definition of $(\vx^{(t)}, \vy^{(t)})$, $\pr_{(i, j) \sim (\vx^{(t)}, \vy^{(t)}) }[i = j] = T/k$ for any $t \in [T]$. So, $\sw(\vx^{(t)} \otimes \vy^{(t)}) = 1 + \gamma T/k$, where we used the fact that $K^{(t)} \subseteq [n]$ forms a clique on $G$ (by construction). In turn, this implies that $\sw(\vmu) = \frac{1}{T} \sum_{t=1}^T \sw(\vx^{(t)} \otimes \vy^{(t)}) = 1 + \gamma T/k$.

    Next, we show that $\vmu$ is a CCE. By symmetry, it suffices to consider deviations of Player $y$. We first observe that the marginal of $\vmu$ with respect to Player $x$, $\frac{1}{T} \sum_{t=1}^T \vx^{(t)}$, is the uniform distribution over the clique $K$. Thus, any deviation of Player $y$ to an action $j \in [n]$ can yield an (expected) utility of at most $\frac{1}{2}(1 + \gamma/k)$; this is at most the utility obtained under $\vmu$, which we saw was $\frac{1}{2}(1 + \gamma T/k)$ (since the players receive the same utility when the game is restricted on $\mat{A}$). Further, any deviation to an action $n+1 \leq j \leq 2n$ can lead to a utility of at most $\frac{1}{2}$. This is again strictly worse than what obtained under $\vmu$ since $\gamma > 0$, completing the proof.
\end{proof}

\badmass*

\begin{proof}
    We define $\delta^{(t)} \defeq 1 - \sum_{i=1}^n \vx_i^{(t)} \sum_{j=1}^n \vy_j^{(t)}$ for each $t \in [T]$. We will first show that $\sum_{t=1}^T \alpha^{(t)} \delta^{(t)} \leq \gamma$. Indeed, we can bound the welfare of each individual product distribution as
    \[
        \sw(\vx^{(t)} \otimes \vy^{(t)}) = \langle \vx^{(t)}, (\mat{R} + \mat{C} ) \vy^{(t)} \rangle = \sum_{i=1}^n \sum_{j=1}^n \vx_i^{(t)} (\mat{A}_{i, j} + \gamma \mathbbm{1} \{ i = j\} ) \vy_j^{(t)} \leq (1 + \gamma) (1 - \delta^{(t)}),
    \]
    by definition of $\mat{R}$ and $\mat{C}$ in~\eqref{eq:game}. Thus, we have
    \[
        1 \leq \sw(\vmu) = \sum_{t=1}^T \alpha^{(t)} \sw(\vx^{(t)} \otimes \vy^{(t)}) \leq (1 + \gamma) \left(1 - \sum_{t=1}^T \alpha^{(t)} \delta^{(t)} \right).
    \]
    So, $\sum_{t=1}^T \alpha^{(t)} \delta^{(t)} \leq \gamma$. We now consider $\Delta^{n} \ni \tilx_{1 \leq i \leq n}^{(t)} = \vx^{(t)}_{1 \leq i \leq n}/\sum_{i=1}^n \vx_i^{(t)}$ and $\Delta^{n} \ni \tily_{1 \leq j \leq n}^{(t)} = \vy^{(t)}_{1 \leq j \leq n}/\sum_{j=1}^n \vy_j^{(t)}$ for all $t \in [T]$. Accordingly, we define $\tilvmu \defeq \sum_{t=1}^T \alpha^{(t)} (\tilx^{(t)} \otimes \tily^{(t)})$; by construction, each product of $\tilvmu$ is supported solely on $[n] \times [n]$. It is also clear that $\sw(\tilvmu) \geq \sw(\vmu)$ since, also by construction, $\tilx_i^{(t)} \geq \vx_i^{(t)}$ and $\tily_j^{(t)} \geq \vy_j^{(t)}$ for all $t \in [T]$ and $(i, j) \in [n] \times [n]$. As a result, it suffices to bound the CCE gap of $\tilvmu$. To that end, we will consider only deviations by Player $x$, as deviations by Player $y$ can be treated similarly. Since $\vmu$ is assumed to be an $\epsilon$-CCE, we have that for any $\hatvx \in \Delta^{2n}$,
    \begin{equation}
        \label{eq:CCE-def}
        \sum_{t=1}^T \alpha^{(t)} \langle \hatvx - \vx^{(t)}, \mat{R} \vy^{(t)}  \rangle \leq \epsilon.
    \end{equation}
    Now, we bound
    \begin{align}
        \langle \vx^{(t)}, \mat{R} \vy^{(t)} \rangle &\leq \sum_{i=1}^n \sum_{j=1}^n \vx_i^{(t)} \mat{R}_{i, j} \vy_j^{(t)} + \sum_{i=n+1}^{2n} \sum_{j=1}^n \vx_i^{(t)} \mat{R}_{i, j} \vy_j^{(t)} \notag \\
        &= \frac{1}{2} \sum_{i=1}^n \sum_{j=1}^n \vx_i^{(t)} (\mat{A}_{i, j} + \gamma \mathbbm{1} \{ i = j \} ) \vy_j^{(t)} + \frac{k}{2} \left( 1 - \sum_{i=1}^n \vx_i^{(t)} \right) \left(\sum_{j=1}^n \vy_j^{(t)} \right) \notag \\
        &\leq \frac{1}{2} \sum_{i=1}^n \sum_{j=1}^n \tilx_i^{(t)} (\mat{A}_{i, j} + \gamma \mathbbm{1} \{ i = j \} ) \tily_j^{(t)} + \frac{k}{2} \left( 1 - \sum_{i=1}^n \sum_{j=1}^n \vx_i^{(t)} \vy_j^{(t)} \right) \notag \\
        &= \langle \tilx^{(t)}, \mat{R} \tily^{(t)} \rangle + \frac{k}{2} \delta^{(t)}.\label{eq:ub-cce}
    \end{align}
Also, for any $\hatvx \in \Delta^{2n}$,
\begin{equation}
    \label{eq:lb-cce}
    \langle \hatvx, \mat{R} \vy^{(t)} \rangle = \langle \hatvx, \mat{R} \tily^{(t)} \rangle - \sum_{i=1}^{2n} \sum_{j=1}^{2n} \hatvx_i \mat{R}_{i, j} (\vy^{(t)}_j - \tily^{(t)}_j) \geq \langle \hatvx, \mat{R} \tily^{(t)} \rangle - k \delta^{(t)},
\end{equation}
where the inequality above uses the fact that $\| \vy^{(t)} - \tily^{(t)} \|_1 = 2 ( 1 - \sum_{j=1}^n \vy_j^{(t)})$. Indeed, when $\sum_{j=1}^n \vy_j^{(t)} = 0$, we have $\| \vy^{(t)} - \tily^{(t)} \|_1 = \|\vy^{(t)} \|_1 + \|\tily^{(t)} \|_1 = 2 = 2 ( 1 - \sum_{j=1}^n \vy_j^{(t)})$; in the contrary case, we have
\begin{align*}
    \|\vy^{(t)} - \tily^{(t)} \|_1 &= \|\vy^{(t)}_{n+1 \leq j \leq 2n} \|_1 + \left\|\vy^{(t)}_{1 \leq j \leq n} - \frac{\vy^{(t)}_{1 \leq j \leq n}}{\sum_{j=1}^n \vy_j^{(t)}} \right\|_1 \\
    &= 1 - \sum_{j=1}^n \vy_j^{(t)} + \left( 1 - \frac{1}{\sum_{j=1}^n \vy_j^{(t)}} \right) \sum_{j=1}^n \vy_j^{(t)} = 2 \left( 1 - \sum_{j=1}^n \vy_j^{(t)} \right).
\end{align*}
Combining~\eqref{eq:ub-cce} and~\eqref{eq:lb-cce} with~\eqref{eq:CCE-def}, it follows that for any $\tilx \in \Delta^{2n}$,
\[
    \sum_{t=1}^T \alpha^{(t)} \langle \hatvx - \tilx^{(t)}, \mat{R} \tily^{(t)} \rangle \leq \epsilon + 2 k \sum_{t=1}^T \alpha^{(t)} \delta^{(t)} \leq \epsilon + 2k \gamma,
\]
and the same bound applies for $\sum_{t=1}^T \alpha^{(t)} \langle \hatvy - \tily^{(t)}, \mat{C}^\top \tilx^{(t)} \rangle$. This shows that $\tilvmu$ is an $(\epsilon + 2k \gamma)$-CCE, as claimed. This completes the proof.
\end{proof}

\smallprob*

\begin{proof}
    Fix some $i \in [n]$. We see that a deviation from Player $y$ to the $n + i$ column would give that player a utility of $\mat{C}_{i, n+i} \left( \sum_{t=1}^T \alpha^{(t)} \vx^{(t)}_i \right)$. But the current utility of Player $y$ under $\vmu$ is at most $\frac{1}{2} (1 + \gamma) $ since $\vmu$ is assumed to be supported only on $[n] \times [n]$. As a result, since $\vmu$ is an $\epsilon'$-CCE, this implies that $k \sum_{t=1}^T \alpha^{(t)} \vx_i^{(t)} \leq (1 + \gamma) + 2 \epsilon'$, which in turn yields
    \[
         \max_{1 \leq t \leq T} \alpha^{(t)} \vx_i^{(t)} \leq \frac{1 + \gamma + 2 \epsilon'}{k}.
    \]
    Similar reasoning gives the same bound on $\max_{ 1 \leq t \leq T} \alpha^{(t)} \vy_j^{(t)}$ for any $j \in [n]$.
\end{proof}

\inducedclique*

Before we proceed with the proof, we will make use of a simple claim stated and proven below.

\begin{claim}
    \label{claim:squared-bound}
    Let $\vx \in \R^{n}$ be such that $0 \leq \vx_i \leq 1/\ell$ for all $i \in [n]$ and $\sum_{i=1}^n \vx_i = p \in (0, n/\ell]$. Then, $\sum_{i=1}^n \vx_i^2 \leq p/\ell$.
\end{claim}

\begin{proof}
    Let $\vx \in \R^n$ be a maximizer of $\sum_{i=1}^n \vx_i^2$ subject to the constraints specified above. Let $S \subseteq [n]$ be the nonzero indexes of $\vx$. For the sake of contradiction, suppose that there exist $i, i' \in S$ with $i \neq i'$ such that $\vx_{i} > \vx_{i'}$ and $\vx_i < 1/\ell$. Then, there is a sufficiently small $\epsilon > 0$ such that $\vx_{i} + \epsilon \leq 1/\ell$ and $\vx_{i'} - \epsilon \geq 0$, and at the same time $(\vx_i + \epsilon)^2 + (\vx_{i'} - \epsilon)^2 > \vx_i^2 + \vx_{i'}^2$. This contradicts the optimality of $\vx$. We conclude that there are two possible cases. First, if $\vx_i = p/|S|$ for all $i \in S$, we have $\sum_{i \in S} \vx_i^2 = p^2/|S| \leq p/\ell$ (since $p/|S| \leq 1/\ell$ by feasibility). Otherwise, there is a coordinate $i \in S$ such that $\vx_i < 1/\ell$ while $\vx_{i'} = 1/\ell$ for $i' \in S \setminus \{i\}$. Thus, $\sum_{i \in S} \vx_i^2 \leq (|S| - 1)/\ell^2 + ( p - (|S| - 1)/\ell)^2 < (|S| - 1)/\ell^2 + ( p - (|S| - 1)/\ell) / \ell = p/\ell$.
\end{proof}

\begin{proof}[Proof of~\Cref{lemma:induced-clique}]
    Given that $\vx \otimes \vy$ is supported only on $[n] \times [n]$, we have
    \[
        (1 + \gamma) \sum_{i=1}^n \vx_i \vy_i + \left(1 - \sum_{i=1}^n \vx_i \vy_i \right) \geq \sw(\vx \otimes \vy) \geq 1 + \gamma / \ell - 6 \gamma^2 T^2,
    \]
    which implies that $\sum_{i=1}^n \vx_i \vy_i \geq 1/\ell - 6 \gamma T^2$. Further, \Cref{claim:squared-bound} implies that $\sum_{i=1}^n \vx_i^2 \leq (1 + 6 k \gamma) /\ell $ and $\sum_{i=1}^n \vy_i^2 \leq (1 + 6 k \gamma) /\ell$. Thus, combining the previous inequalities,
    \begin{equation}
        \label{eq:dist-xy}
        \|\vx - \vy \|^2 = \sum_{i=1}^n \vx_i^2 + \sum_{i=1}^n \vy_i^2 - 2 \sum_{i=1}^n \vx_i \vy_i \leq \frac{12 k \gamma + 12 \gamma T^2 }{\ell} \leq \frac{15 k^2 \gamma}{\ell} .
    \end{equation}
    Moreover,
    \begin{align*}
        \frac{1}{\ell} \leq \langle \vx, \vy \rangle = \langle \vx, \vy - \vx \rangle + \|\vx\|^2 &\leq \|\vx\| \|\vx - \vy\| + \|\vx\|^2 \\
        &\leq \sqrt{ \frac{1 + 6 k \gamma}{\ell}} \sqrt{\frac{15 k^2 \gamma}{\ell}} + \|\vx\|^2 \\
        &\leq \frac{4 k \sqrt{\gamma}}{\ell} + \|\vx\|^2
    \end{align*}
    since $\sqrt{1 + 4 k \gamma} \leq \sqrt{16/15}$. Rearranging,
    \begin{equation}
        \label{eq:lb-x2norm}
        \|\vx\|^2 \geq \frac{1}{\ell} \left( 1 - 4 k \sqrt{\gamma}\right).
    \end{equation}
Now, let $S \defeq \{i \in [n] : \vx_i \geq (1 - \gamma')/\ell \}$ for $\gamma' \defeq 40 \ell^2 k \sqrt{\gamma}$, and $p \defeq \sum_{i \in S} \vx_i$. Applying~\Cref{claim:squared-bound} to both $S$ and $[n] \setminus S$,
\[
     \|\vx\|^2 = \sum_{i \in S} \vx_i^2 + \sum_{ i \in [n] \setminus S} \vx_i^2 
     \leq p \frac{1 + 6 k \gamma}{\ell} + (1 -p) \frac{1 - \gamma'}{\ell}.
\]
Combining with~\eqref{eq:lb-x2norm}, we get
\[
     p \geq \frac{\gamma' - 4 k \sqrt{\gamma} }{6 k \gamma + \gamma'} \geq 1 - \frac{1}{4 \ell^2},
\]
where we used that $\gamma' = 40 \ell^2 k \sqrt{\gamma}$. We now claim that $|S| = \ell$. Indeed, since $(1 - \gamma')/\ell \leq \vx_i \leq (1 + 6 k \gamma) /\ell$ for all $i \in S$, we have
\[
    \frac{1 - \gamma'}{\ell} |S| \leq \sum_{i \in S} \vx_i \leq 1 \implies |S| \leq \frac{\ell}{1 - \gamma'} = \frac{\ell}{ 1 - 40 \ell^2 k \sqrt{\gamma} } < \ell + 1
\]
for $\gamma < \frac{1}{40^2 \ell^4 (\ell+1)^2 k^2}$, and (since $p = \sum_{i \in S} \vx_i \geq 1 - 1/(4 \ell^2)$)
\[
    1 - \frac{1}{4 \ell^2} \leq \sum_{i \in S} \vx_i \leq |S| \frac{1 + 6 k \gamma}{ \ell} \implies |S| > \ell - 1.
\]
Thus, $|S| = \ell$. We now show that $S$ is an $\ell$-clique on $G$. We first note that, by~\eqref{eq:dist-xy},
\[
  \vy_j \geq \vx_j - \sqrt{ \frac{15 k^2 \gamma}{\ell}} \geq \frac{1 - \gamma'}{\ell} - 4 k \sqrt{\frac{\gamma}{\ell}}  \geq \frac{1}{\ell} - \frac{1.5}{\ell(\ell+1)} \geq \frac{1}{2\ell}
\] 
 for all $j \in S$, where the penultimate inequality follows from our choice of $\gamma$ and $\gamma'$, and the last inequality uses that $\ell \geq 2$. If we assume for the sake of contradiction that there exist $i', j' \in S$ such that $\mat{A}_{i', j'} = 0$, that is, $S$ is not a clique on $G$, then
 \begin{align*}
     \sw(\vx \otimes \vy) &= \sum_{i=1}^n \sum_{j = 1}^n \vx_i (\mat{A}_{i, j} + \gamma \mathbbm{1} \{ i = j \} ) \vy_j \\ &\leq (1 + \gamma) \sum_{i=1}^n \vx_i \vy_i + \sum_{i=1}^n \sum_{j \neq i} \mathbbm{1} \{\{i, j\} \neq \{i', j'\}\} \vx_i \mat{A}_{i, j} \vy_j + 2 
\vx_{i'} \mat{A}_{i', j'} \vy_{j'} \\ &\leq (1 + \gamma) \frac{1 + 6 k \gamma}{\ell} + 1 - \frac{1 + 6 k\gamma}{\ell} - \frac{1}{2 \ell^2} \\
     &\leq 1 + \frac{\gamma}{\ell} - \frac{1}{\ell^2} < 1 + \frac{\gamma}{\ell} - 6 \gamma^2 T^2,
 \end{align*}
 where the last inequality follows from the choice of $\gamma$. This is a contradiction since $\sw(\vx \otimes \vy) \geq 1 + \gamma/\ell - 6 \gamma^2 T^2$.
 \end{proof}

We are now ready to combine the previous pieces in order to prove~\Cref{theorem:algorithm1}. 

\begin{proof}[Proof of~\Cref{theorem:algorithm1}]
    It suffices to show that if $G$ contains a $k$-clique, then~\Cref{line:S} outputs a $k/T$-clique. Indeed, if $\omega(G) \leq 2 T$, then~\Cref{alg:maxclique} trivially returns a $2T$-approximation; otherwise, it suffices to consider the largest iteration of the algorithm such that $k \leq \omega(G)$. Consider now for that iteration the $T$-sparse $\epsilon$-CCE, $\vmu = \sum_{t=1}^T \alpha^{(t)} (\vx^{(t)} \otimes \vy^{(t)})$, given as output by $\sparsecce$ in~\Cref{line:sparsecce}; we can assume here that $\alpha^{(t)} > 0$ for all $t \in [T]$. Let $\tilvmu \defeq \sum_{t=1}^T \alpha^{(t)} (\tilx^{(t)} \otimes \tily^{(t)})$, where $(\tilx^{(t)})_{1 \leq t \leq T}$ and $(\tily^{(t)})_{1 \leq 
t \leq T}$ are as in~\Cref{line:til}. By~\Cref{lemma:optimalCCE}, we know that there is a $T$-sparse CCE with welfare at least $1 + \gamma T/k$, and so since the optimality gap $\epswel$ is small enough (\Cref{line:eps}) we get that $\sw(\vmu) \geq 1$. Thus, we can apply~\Cref{lemma:bad-mass} to conclude that $\tilvmu$ is an $(\epsilon + 2k \gamma)$-CCE, which is a $(5 k \gamma /2)$-CCE by our choice of $\epsilon$ (\Cref{line:eps}). Next, \Cref{lemma:small-prob} implies that $\tilx_i^{(t)} \leq (1 + \gamma + 5 k \gamma)/(\alpha^{(t)} k)$ for all $i \in [n]$ and $t \in [T]$. Using~\Cref{claim:squared-bound} and Cauchy-Schwarz, we have
\[
    \sum_{i=1}^n \tilx_i^{(t)} \tily_i^{(t)} \leq \sqrt{ \left( \sum_{i=1}^n (\tilx_i^{(t)})^2 \right) \left( \sum_{i=1}^n (\tily_i^{(t)})^2 \right) } \leq \frac{1 + \gamma + 5 k \gamma}{\alpha^{(t)} k }.
\]
Thus, for all $t \in [T]$,
\begin{equation}
    \label{eq:sw-bound}
    \sw(\tilx^{(t)} \otimes \tily^{(t)}) \leq 1 + \frac{\gamma + \gamma^2 + 5 k \gamma^2}{\alpha^{(t)} k}.
\end{equation}
By~\Cref{lemma:optimalCCE,lemma:bad-mass}, we have
\begin{align}
    \alpha^{(t)} \sw(\tilx^{(t)} \otimes \tily^{(t)}) &\geq 1 + \frac{\gamma T}{k} - \epswel - \sum_{\tau \neq t} \alpha^{(\tau)} \sw(\tilx^{(\tau)} \otimes \tily^{(\tau)}) \notag \\
    &\geq \alpha^{(t)} + \frac{\gamma T}{k} - \epswel - (T-1) \frac{\gamma + \gamma^2 + 5 k \gamma^2}{k} \label{align:sw-bound} \\
    &\geq \alpha^{(t)} + \frac{\gamma}{k} - 5 \gamma^2 T - \frac{T}{k} \gamma^2 - \epswel \geq \alpha^{(t)} + \frac{\gamma}{k} - 6 \gamma^2 T, \label{align:epswel}
\end{align}
where~\eqref{align:sw-bound} uses~\eqref{eq:sw-bound} and the fact that $\alpha^{(t)} = 1 - \sum_{\tau \neq t} \alpha^{(\tau)} $, and~\eqref{align:epswel} follows from our choice of $\epswel$ and the fact that $k \geq 2$. Now, let $t^\star \in [T]$ be such that $\alpha^{(t^\star)} \geq 1/T$; \Cref{line:tstar} returns such a $t^\star$. Then, \eqref{align:epswel} implies that $\sw(\tilx^{(t^\star)} \otimes \tily^{(t^\star)}) \geq 1 + \frac{\gamma}{\alpha^{(t^\star)} k} - 6 \gamma^2 T^2$ since $\alpha^{(t^\star)} \geq 1/T$. Finally, we can use \Cref{lemma:induced-clique} with respect to $\tilx^{(t^\star)} \otimes \tily^{(t^\star)}$ to obtain an $(\alpha^{(t^\star)} k)$-clique, and thereby a $k/T$-clique in $G$ since $\alpha^{(t^\star)} \geq 1/T$. This completes the proof.
\end{proof}


\subsection{Proof of Theorem~\ref{theorem:uniqueness}}
\label{appendix:proof2}

We next provide the proof of~\Cref{theorem:uniqueness} pertaining to the computational complexity of $\uniquesparsecce$, restated below.

\uniqueness*

We will use the fact that distinguishing whether an $n$-node graph $G$ has a clique of size at most $n^{\epsilon}$ or at least $n^{1 - \epsilon}$ is \NP-hard for any $\epsilon > 0$~\citep{Zuckerman07:Linear}. We proceed as follows. We augment the game given in~\eqref{eq:game} with an additional action, say $\newaction$, for each player. We will refer to the resulting game as $\cG'$. When both players select $\newaction$, they both receive a utility of $r \defeq (1 + \gamma T/k)/2$. When only one player selects $\newaction$, that player receives $r$ while the other player receives $-r$. It is clear that $(\newaction, \newaction)$ is a (pure) Nash equilibrium, and hence a $T$-sparse CCE. Moreover, \Cref{lemma:optimalCCE} shows that when $G$ contains a $k$-clique, there is a uniform $T$-sparse correlated distribution $\vmu$ supported only on the $n \times n$ submatrix corresponding to $\mat{A}$, in which each player obtains a utility of $r$. It is easy to see that $\vmu$ is a $T$-sparse CCE in the new game as well. What remains to show thus is that when $G$ does not contain an $\Omega(k/T)$ clique, $(\newaction, \newaction)$ is the only uniform $T$-sparse CCE of $\cG'$.

Indeed, since a player can always switch to playing $\newaction$, which secures that player a utility of $r$, any $T$-sparse CCE in $\cG'$ must have welfare at least $2r = 1 + \gamma T / k$. Following the argument of~\Cref{subsec:prooftheorem}, when $\gamma$ is sufficiently small, we will show that this can only happen under $(\newaction, \newaction)$ or when $G$ contains an $\Omega(k/T)$-clique. In proof, let $\vmu = \frac{1}{T} \sum_{t=1}^T \vx^{(t)} \otimes \vy^{(t)}$ be a CCE in $\cG'$ distinct from $(\newaction, \newaction)$, which we argued must satisfy $\sw(\vmu) \geq 1 + \gamma T / k$. We consider now the product $t \in [T]$ that maximizes $\sw(\vx^{(t)} \otimes \vy^{(t)})$ subject to the constraint that the probability mass assigned to the $n \times n$ submatrix corresponding to $\mat{A}$ is (strictly) positive. It is clear that $\sw(\vx^{(t)} \otimes \vy^{(t)}) \geq 1 + \gamma T/k$. We will now argue that $p \defeq \pr_{i \sim \vx^{(t)}, j \sim \vy^{(t)}} [i \leq n, j \leq n ] \geq 1 - 2\gamma$. Let $p_{\newaction} = \pr_{i \sim \vx^{(t)}, j \sim \vy^{(t)}} [i = \newaction, j = \newaction]$. Then, it follows that $\sw(\vx^{(t)} \otimes \vy^{(t)}) \leq p (1 + \gamma) + p_{\newaction} (1 + \gamma T /k)$ since $\cG'$ is, by construction, zero-sum when excluding $(\newaction, \newaction)$ and the $n \times n$ submatrix corresponding to $\mat{A}$. Thus, $p + p_{\newaction} \geq 1 - \gamma$. Further, a union bound implies that $p + p_{\newaction} + 2 p p_{\newaction} \leq 1$. Indeed, we have
\begin{align*}
    \pr_{i \sim \vx^{(t)}, j \sim \vy^{(t)}} [i = \newaction, j \neq \newaction] &= \pr_{i \sim \vx^{(t)}} [i = \newaction] \pr_{j \sim \vy^{(t)}} [j \neq \newaction] \\
    &\geq \pr_{i \sim \vx^{(t)}, j \sim \vy^{(t)}} [i = \newaction, j = \newaction] \pr_{i \sim \vx^{(t)}, j \sim \vy^{(t)}} [i \leq n, j \neq \newaction]  \\
    &\geq p_{\newaction} p,
\end{align*}
and the same lower bound applies to $\pr_{i \sim \vx^{(t)}, j \sim \vy^{(t)}} [i \neq \newaction, j = \newaction]$. Combining with the fact that $\sw(\vx^{(t)} \otimes \vy^{(t)}) \geq 1 + \gamma T/k$, we conclude that
\[
    1 + \gamma \frac{T}{k} \leq 1 - 2 p p_{\newaction} + p \gamma + p_{\newaction} \gamma \frac{T}{k} \leq 1 + \gamma \frac{T}{k} - 2 p p_{\newaction} + p \gamma \implies p_{\newaction} \leq \gamma,
\]
where we used that $p > 0$. Next, we define $\Delta^n \ni \tilx_{1 \leq i \leq n}^{(t)} =  \nicefrac{\vx^{(t)}_{1 \leq i \leq n}}{\sum_{i=1}^n \vx_i^{(t)}}$ and $\Delta^n \ni \tily_{1 \leq i \leq n}^{(t)} =  \nicefrac{\vy^{(t)}_{1 \leq i \leq n}}{\sum_{i=1}^n \vy_i^{(t)}}$. Similarly to~\Cref{lemma:small-prob}, we now have that $\tilx_{i}^{(t)}, \tily_j^{(t)} \leq 2/\ell$ for any $(i, j) \in [n] \times [n]$, where $\ell \defeq k/T$ and $\gamma$ is sufficiently small. Indeed, under $\vmu$ each player secures a utility of at least $1/2$; since $\vmu$ is also assumed to be a CCE, considering the deviation of Player $y$ to column $n + i$ we have that for any $i \in [n]$,
\[
    \frac{1}{2} \geq \frac{k}{2T} \vx_i^{(t)} - \frac{T-1}{T} r \implies \tilx_i^{(t)} \leq \frac{2}{\ell}
\]
when $\gamma$ is sufficiently small, where we used the fact that $\sum_{i=1}^n \vx_i^{(t)} \geq p \geq 1 - 2 \gamma$. Similar reasoning yields that $\tily_j^{(t)} \leq 2/\ell$ for any $j \in [n]$. Moreover, we know that $\sw(\tilx^{(t)} \otimes \tily^{(t)}) \geq 1 + \gamma/\ell$, which in turn implies that $\sum_{i=1}^n \tilx_i^{(t)} \tily_i^{(t)} \geq 1/\ell$. To conclude the argument, we will show---analogously to~\Cref{lemma:induced-clique}---how to extract an $\Omega(\ell)$-clique from that product distribution. Namely, we identify the set $S$ consisting of all $i \in [n]$ such that $\tilx_i, \tily_i \geq 1/(16 \ell)$. Then,
\begin{align}
    \frac{1}{\ell} \leq \sum_{i=1}^n \tilx_i^{(t)} \tily_i^{(t)} &= \sum_{i \in S} \tilx_i^{(t)} \tily_i^{(t)} + \sum_{i \notin S} \tilx_i^{(t)} \tily_i^{(t)} \\
    &= \sum_{i \in S} \tilx_i^{(t)} \tily_i^{(t)} + \sum_{i \notin S} \max(\tilx_i^{(t)}, \tily_i^{(t)}) \min (\tilx_i^{(t)}, \tily_i^{(t)}) \\
    &\leq |S| \frac{4}{\ell^2} + \sqrt{ \sum_{i \notin S} \max(\tilx_i^{(t)}, \tily_i^{(t)})^2 \sum_{i \notin S} \min ( \tilx_i^{(t)}, \tily_i^{(t)})^2 } \label{align:bound-maxmin} \\
    &\leq |S| \frac{4}{\ell^2} + \sqrt{ \frac{4}{\ell} \frac{1}{16 \ell}},\label{align:claim-bound}
\end{align}
where~\eqref{align:bound-maxmin} uses the Cauchy-Schwarz inequality and the fact that $\tilx_i^{(t)}, \tily^{(t)}_i \leq 2/\ell$, and~\eqref{align:claim-bound} is a consequence of~\Cref{claim:squared-bound}; to apply~\Cref{claim:squared-bound}, we note that $\sum_{i \notin S} \max(\tilx_i^{(t)}, \tily_i^{(t)}) \leq \sum_{i \notin S} ( \tilx_i^{(t)} + \tily_i^{(t)}) \leq 2$; $\sum_{i \notin S} \min(\tilx_i^{(t)}, \tily_i^{(t)}) \leq \sum_{i \notin S} \tilx_i^{(t)} \leq 1$; $\max(\tilx_i^{(t)}, \tily_i^{(t)}) \leq 2/\ell$ for all $i \in [n]$; and $\min(\tilx_i^{(t)}, \tily_i^{(t)}) \leq 1/(16\ell)$ for all $i \in [n] \setminus S$ (by definition of $S$). As a result, we conclude that $|S| \geq \ell/8$. Finally, similarly to the argument of~\Cref{lemma:induced-clique}, it is easy to see that $S$ induces a clique on $G$; the contrary case would contradict the fact that $\sw(\tilx^{(t)} \otimes \tily^{(t)}) \geq 1 + \gamma/\ell$.

Therefore, under uniqueness we know that $G$ does not contain a clique of size $k$, while in the contrary case $G$ must contain a clique of size $\Omega(k/T)$. Taking $k = n^{1 - \epsilon}$ and $T = \Omega(n^{1 - 2 \epsilon})$ in conjunction with the result of~\citet{Zuckerman07:Linear} leads to~\Cref{theorem:uniqueness}.

As we explained earlier, it is not clear how to show hardness when we allow non-uniform mixtures. In particular, taking two mixtures on $(1, 1)$ and $(\newaction,\newaction)$ and weights $\alpha^{(1)}$, $\alpha^{(2)}$ with $\alpha^{(1)} \approx 0$ is a ($2$-sparse) CCE for $\cG'$, but clearly does not contain any useful information about $G$.

\fi

\subsection{Proof of Theorem~\ref{theorem:constant}}
\label{appendix:proof3}

Finally, we provide the proof of~\Cref{theorem:constant}, which is restated below.

\constant*

The proof mostly follows the argument of~\citet{Hazan11:How}. Similarly to~\eqref{eq:game}, we consider a two-player game defined by the payoff matrices
\begin{equation}
    \label{eq:Hazangame}
    \R^{N \times N} \ni \mat{R} \defeq 
    \frac{1}{2}  
    \begin{pmatrix}
       \mat{A} & - \mat{B}^\top \\
        \mat{B} & \mat{0}_{N - n}
    \end{pmatrix}
    \text{ and }
    \R^{N \times N} \ni \mat{C} \defeq
    \frac{1}{2} 
    \begin{pmatrix}
       \mat{A} & \mat{B}^\top \\
        - \mat{B} & \mat{0}_{N-n}
    \end{pmatrix},
\end{equation}
where $N$ is sufficiently large, $\mat{A}$ is again the \emph{adjacency} matrix (with $1$ on the diagonal entries) of $G$---the input of the planted clique problem, and $\mat{B} \in \R^{(N - n) \times n}$ is defined by selecting each entry independently as
\[
    \mat{B}_{i, j} =
    \begin{cases}
        M & \text{with probability } \frac{3}{4} \frac{1}{M} \text{ and }\\
        0 & \text{otherwise},
    \end{cases}
\]
where $M = M(n)$ is sufficiently large. We first note that game~\eqref{eq:Hazangame} admits, with high probability, a Nash equilibrium with welfare $1$. In what follows, we recall that $k \in \N$ represents the size of the planted clique.

\begin{lemma}
    Consider game~\eqref{eq:Hazangame} with $k \geq 32 M^2 ( \log N - 2 \log n)$. Then, with high probability there is a Nash equilibrium with welfare $1$.
\end{lemma}

\begin{proof}
    We consider the strategy profile $(\vx, \vy)$ in which both players play uniformly at random over the nodes corresponding to the planted clique. It is clear that $\sw(\vx \otimes \vy) = 1$. It thus suffices to show that $(\vx, \vy)$ is indeed a Nash equilibrium of~\eqref{eq:Hazangame}. By symmetry, we can analyze only deviations of Player $x$. When $i \leq n$, it is clear that there is no profitable deviation for Player $x$ as that player obtains $1/2$ under $(\vx, \vy)$, which is the highest utility attainable in the $n \times n$ submatrix corresponding to $\mat{A}$. Let us consider thus some $i > n$. The obtained utility then is half the average over $k$ entries of $\mat{B}$, which is highly concentrated around $3/4$---the mean value. In particular, by a Chernoff–Hoeffding bound, it follows that the probability that $i$ is profitable is upper bounded by $e^{- \frac{k^2}{32 M^2}}$. Thus, by a union bound, the probability that there is a profitable deviation among $i > n$ is upper bounded by $(N-n) e^{- \frac{k^2}{32 M^2}} \leq 1/n^2$, where we used the assumption that $k \geq 32 M^2 (\log N - 2 \log n)$. This completes the proof.
\end{proof}

\begin{lemma}
    \label{lemma:bad-mass-new}
    Given a $T$-sparse $\epseq$-CCE of~\eqref{eq:Hazangame} with welfare $1 - \epswel$, we can compute in polynomial time an $(\epseq+ 2M T \epswel)$-CCE with welfare at least $1 - \epswel$ and supported only on $[n] \times [n]$.
\end{lemma}

The proof of this lemma is similar to that of~\Cref{lemma:bad-mass}. In particular, we define $\delta^{(t)} = 1 - \sum_{i=1}^n \vx_i^{(t)} \sum_{j=1}^n \vy_j^{(t)}$ for each $t \in [T]$. Then, 
\[
1 - \epswel \leq \sum_{t=1}^T \alpha^{(t)} \sw(\vx^{(t)} \otimes \vy^{(t)}) = \sum_{t=1}^T \alpha^{(t)} \sum_{i=1}^n \sum_{j=1}^n \vx_i^{(t)} \mat{A}_{i, j} \vy_j^{(t)} \leq 1 - \sum_{t=1}^T \alpha^{(t)} \delta^{(t)},
\]
in turn implying that $\sum_{t=1}^T \alpha^{(t)} \delta^{(t)} \leq \epswel$. The rest of the argument then is the same as in~\Cref{lemma:bad-mass}. Next, the lemma below gives a bound analogous to~\Cref{lemma:small-prob}. (In what follows, we can safely assume that $c_2 \log n$ is an integer.)

\begin{lemma}
    \label{lemma:near-uni}
    Let $\vmu = \sum_{t=1}^T \alpha^{(t)} (\vx^{(t)} \otimes \vy^{(t)})$
    be a $\frac{1}{2}$-CCE of~\eqref{eq:Hazangame} such that each $\vx^{(t)} \otimes \vy^{(t)}$ is supported only on $[n] \times [n]$. If $N = n^{c_1}$ and $c_1  - c_2 \log (4M/3) = 2$, then with high probability the probability mass every player places on every set of $c_2 \log n$ pure strategies of the $t$th product distribution is at most $2/(M \alpha^{(t)})$.
\end{lemma}

\begin{proof}
    Let $d \defeq c_2 \log n$. Suppose that Player $y$ places on some set of $c_2 \log n$ pure strategies of the $t$th product distribution more than $2/(M \alpha^{(t)})$ probability mass. We will compute the probability that there is a row of $\mat{B}$ in which all entries corresponding to $d$ have a value of $M$. If that event happens, Player $x$ can deviate to that row and obtain a utility larger than $1$, while the current utility is at most $1/2$. The probability that event occurs for a single row is $p^d$ for $p = \frac{3}{4M}$, and there are $N-n$ rows which are independent. Thus, the probability that no such rows exists reads 
    \[
        (1 - p^d)^{N - n} \leq e^{-\frac{n^2}{2}},
    \]
    where we used the assumption that $N = n^{c_1}$ and $c_1 - c_2 \log(4M/3) = 2$. Finally, we can rule out all sets with size $c_2 \log n$ via a union bound, leading to the statement.
\end{proof}

In the lemma below, the density $\dens(S, T)$ of sets $S, T \subseteq [n]$ with $|S| = |T|$ is the probability that an edge exists (with self-loops included) between two nodes chosen uniformly at random from $S$ and $T$.

\begin{lemma}
    \label{lemma:bipartite}
    Given a $\frac{1}{2}$-CCE of~\eqref{eq:Hazangame} supported only on $[n] \times [n]$ and with welfare at least $1 - \epswel$, we can find in polynomial time sets $S, T \subseteq [n]$ with $ |S| = |T| = c_2 \log n$ and $\dens(S, T) \geq \frac{3}{5}$, assuming that $M > 4 T$ and $\epswel \leq 1/(10T)$.
\end{lemma}

\begin{proof}
    Let $\vmu = \sum_{t=1}^T \alpha^{(t)} (\vx^{(t)} \otimes \vy^{(t)})$. We select any $t \in [T]$ such that $\alpha^{(t)} \geq 1/T$. Since it is assumed that $\vmu$ has welfare at least $1 - \epswel$, it follows that
    \[
        \langle \vx^{(t)}, \mat{A} \vy^{(t)} \rangle \geq \frac{1}{\alpha^{(t)}} \left( \sw(\vmu) - \sum_{\tau \neq t} \alpha^{(\tau)} \sw(\vx^{(\tau)} \otimes \vy^{(\tau)}) \right) \geq 1 - \delta,
    \]
    where $\delta = \epswel T$. Let $I_y^{(t)} \defeq \{ j : \supp(\vy^{(t)}) : \langle \vx^{(t)}, \mat{A} \vec{e}_j \rangle \} \geq \frac{4}{5}$, where $\vec{e}_j$ is the $j$th unit vector. Then, $\sum_{j \in I_y^{(t)}} \vy_j^{(t)} \geq 1 - 5 \delta$, for otherwise $\langle \vx^{(t)}, \mat{A} \vy^{(t)} \rangle < (1 - 5 \delta) + (5 \delta) \frac{4}{5} = 1 - \delta$. Using the fact that $\epswel \leq 1/(10T) < 1/(5T) - 2/(5M)$ (since $M > 4 T$), it follows that $\sum_{j \in I_y^{(t)}} \vy_j^{(t)} > 2T/M \geq 2/(M\alpha^{(t)})$. As a result, \Cref{lemma:near-uni} tells us that 
    $|I_y^{(t)}| \geq c_2 \log n$. If $|I_y^{(t)}| > c_2 \log n$, we let $I_y^{(t)}$ be an arbitrary subset of $I_y^{(t)}$ with size $c_2 \log n$. We let $\vec{u}(I_x^{(t)})$ be the uniform distribution on $I_y^{(t)}$. Then, we have
    \[
        \langle \vx^{(t)}, \mat{A} \vec{u}(I_y^{(t)}) \rangle \geq \frac{4}{5}.
    \]
    Similarly, we define $I_x^{(t)} \defeq \{ i \in \supp(\vx^{(t)}) : \langle \vec{e}_i, \mat{A} \vec{u}(I_y^{(t)}) \rangle \geq \frac{3}{5} \}$. Then, $\sum_{ i \in I_x^{(t)} } \vx_i^{(t)} \geq \frac{1}{2} > 2 T/M$ (since $M > 4 T$). Thus, \Cref{lemma:optimalCCE} implies that $|I_x^{(t)}| \geq c_2 \log n$. If $|I_x^{(t)}| > c_2 \log n$, we let $I_x^{(t)}$ be an arbitrary subset of $I_x^{(t)}$ with size $c_2 \log n$. Thus, we have found sets $I_x^{(t)}, I_y^{(t)} \subseteq [n]$ with $|I_x^{(t)}| = |I_y^{(t)}| = c_2 \log n$ and
    \[
        \langle \vec{u}(I_x^{(t)}), \mat{A} \vec{u}(I_y^{(t)}) \rangle \geq \frac{3}{5};
    \]
    that is, $\dens(I_x^{(t)}, I_y^{(t)}) \geq \frac{3}{5}$.
\end{proof}

We finally conclude by stating a lemma shown by~\citet{Hazan11:How}.

\begin{lemma}[\nakedcite{Hazan11:How}]
    \label{lemma:Hazan-dens}
    Given sets $S, T \subseteq [n]$ with $|S| = |T| = 2000 \log n$ and $\dens(S, T) \geq \frac{3}{5}$, we can find in polynomial time a clique of size $100 \log n$ with high probability.
\end{lemma}

As a result, \Cref{theorem:constant} follows from~\Cref{lemma:Hazan-dens,lemma:bipartite,lemma:near-uni,lemma:bad-mass-new,lemma:smallk} using the following choice of parameters:

\begin{itemize}
    \item $k \defeq \lceil 32 M^2 (\log N - \log n) \rceil$;
    \item $M = 5 T$;
    \item $c_2 = 2000$;
    \item $c_1 = c_2 \log (4M/3) + 2$;
    \item $\epswel = \epseq/(4MT)$; and
    \item $\epsilon = 1/4$.
\end{itemize}
